A Train Status Assistant for Indian Railways

Trains are part-and-parcel of every day lives in countries with large, diverse, multi-lingual population like India. Consequently, an assistant which can accurately predict and explain train delays will help people and businesses alike. We present a novel conversation agent which can engage with people about train status and inform them about its delay at in-line stations. It is trained on past delay data from a subset of trains and generalizes to others.

==> background.tex <==
% --------------------
\section{Background}
\label{sec:back}

\subsection{Preliminaries - Dialog and Generating Response with Learning and Reasoning}

A {\em dialog} is made up of a series of {\em turns}, where each turn is a series of {\em utterances} by one or more participants playing one or more {\em roles}. We will assume a customer support setting where the roles are {\em customer} and {\em support agent}.

[Add related work on learning dialog policies]

[Add related work on reasoning/ slot filling dialogs]
% In the example of customer support center, a user contacts a service center and enters into a dialog with a customer support agent. The participant roles here are that of a customer and an agent, and the roles inter-leave in every turn. On the other hand, in the example of online support, a person may raise an issue on a public portal and anyone may reply. 



% --------------------
\subsection{Example - Using Dialogs to Find Information Arranged in a Taxonomy}

One popular category of user dialogs in business setting is inquiry of information that is organized in a taxonomy. For instance, a person wants to ask about a product on a company's site (e.g., {\em pliers} - product, job openings) but does not know which particular type. An example of taxonomy is
United Nations Standard Products and Services Code (UNSPSC\footnote{https://www.unspsc.org/}), which {\em "is an open, global, multi-sector standard for efficient, accurate classification of products and services"}. Table~\ref{tab:unspsc} gives a summary of the levels in the taxonomy and its data. There are 4,302 items arranged into class, family, segment and commodity (lowest level). The {\em characteristic} column conveys the nature of abstraction across levels by reporting number of distinct (dissimilar) values, unique (count=1) values and their percentage, followed by highest frequency at a given level. 

So, if the user inquires about a product, the chatbot can refer to the taxonomy to confirm what the user wants. As example,  a query on   {\em pliers} may refer to a surgical tool (Code: 42292303) or a vehicle servicing equipment (Code: 25191716) or a hand tool (Code: 27112106), and many variations therein. Thus, there can be a varieties strategies for a chatbot to help the user. It can go from highest level to lowest, or reverse, or ask randomly from the tree. Furthermore, if there is a restriction on how many turns the chatbot can take on this query, we want to explore if there are  querying strategies that are optimal.
 

% Distinct means the number of dissimilar values contained for the selected attribute. Unique means the number and percentage of instances having a value for this attribute that no other instances have in the data.


% ---------------------

\begin{table}[t!]
\scriptsize
\centering
\begin{tabular}{|l|l|l|}
\hline
\textbf{Level} & \textbf{Name} & \textbf{Characteristic} \\ \hline
\textbf{4 - Highest} & Segment & 36; 3 (0\%); 825  \\ \hline
\textbf{3} & Family & 173; 23 (1\%); 443  \\ \hline
\textbf{2} & Class & 826; 216 (5\%); 49  \\ \hline
\textbf{1 - Lowest} & Commodity & 4302; 4302 (100\%); 1  \\ \hline
\end{tabular}
\caption{Levels in UNSPSC Taxonomy.}
\label{tab:unspsc}
\end{table}
% ---------------------

% --------------------
\subsection{Related Work}

Conversational interface is considered especially suitable for feature or preference elicitation for at least two reasons~\cite{brennan1990conversation}. First, it is naturally interactive and thus users are more willing to provide additional information. Moreover, it can pro-actively and dynamically channel the information querying process in desired directions. 

Suppose there are $m$ items described using
$n$ features, $F_1$, .., $F_n$. To narrow down users' queries, previous work 
has explored asking to confirm (Yes/No) clarification questions such as ``\textit{are you asking about topic X}''~\cite{horvitz1999computational}, and specify values for a feature by direct inquiry (e.g., ``\textit{What VALUE would you like for FEATURE X"}'')
or multi-choice questions (e.g.``\textit{choices for FEATURE X are VALUE 1... VALUE N''})~\cite{chu2000mimic}. 
We will assume that the features are binary. 
The expected number of features that the user would report in answering a question is $\lambda_{NF}$, the recall rate of the NLP system is $R_{nlp}$, and each unknown feature's information gain is $IG$. 

Such a setting can be used to model an online store selling shirts and trousers (i.e., items) to users. The features can be color, fabric and price category.  A person searching the store may have preferences about fabric and constraints about color when they are buying items together.


% --------------------


==> backup.tex <==
\section{Backup Text - To Remove Later}


In this paper we present the details of the prototype which addresses above-mentioned drawbacks. Below points outline our contributions:

\begin{enumerate}
\item We present a web accessible application which provides delay insights of trains in India (having one of the largest train networks in world) with weeks or months ahead of journey. The predicted delays at in-line stations can quench all of the above-mentioned queries of a consumer.

\item Conversation is a hallmark of intelligence, and consequently, businesses wanting to build AI-based systems to increase productivity and improve customer experience, are interested in automated dialog systems. Therefore along with REST APIs (which enable a machine to communicate with our application), we consider a general chat-bot that can work with learned models and interact with a human.

\item We discuss applicable AI methods like RNNs and LSTMs which can help in predicting more accurate delays and capturing the dynamics of a rail network.
\end{enumerate}
